The giant outburst of 4U 0115+634 in 2011 with Suzaku and RXTE

We present an analysis of X-ray spectra of the high mass X-ray binary 4U 0115+634 as observed with Suzaku and RXTE in 2011 July, during the fading phase of a giant X-ray outburst. We used a continuum model consisting of an absorbed cutoff power-law and an ad-hoc Gaussian emission feature centered around 8.5 keV, which we discuss to be due to cyclotron emission. Our results are consistent with a fundamental cyclotron absorption line centered at ${\sim}10.2$ keV for all observed flux ranges. At the same time we rule out significant influence of the 8.5 kev Gaussian on the CRSF parameters, which are not consistent with the cyclotron line energies and depths of previously reported flux-dependent descriptions. We also show that some continuum models can lead to artificial line-like residuals in the analyzed spectra, which are then misinterpreted as unphysically strong cyclotron lines. Specifically, our results do not support the existence of a previously claimed additional cyclotron feature at ${\sim}15$ keV. Apart from these features, we find for the first time evidence for a He-like Fe XXV emission line at ${\sim}6.7$ keV and weak H-like Fe XXVI emission close to ${\sim}7.0$ keV.

==> linefluxes.tex <==

\multicolumn{5}{l}{this work}\\
\quad absolute$^{a}$
 & $125^{+16}_{-15}$ & -- & $32^{+9}_{-9}$ & $\le 12$  \\
\quad relative$^{b}$
 & $3.1^{+0.4}_{-0.4}\,\%$ & -- & $0.80^{+0.22}_{-0.21}\,\%$ & $\le 0.29\,\%$  \\
\quad residual$^{c}$
 & $88.5^{+1.4}_{-1.5}\,\%$ & -- & $83^{+5}_{-5}\,\%$ & $\ge 87\,\%$  \\
\multicolumn{5}{l}{\citet{Iyer2015a}}\\
\quad absolute$^{a}$
 & $95^{+14}_{-15}$ & $2000^{+700}_{-600}$ & $3300^{+1000}_{-900}$ & $210^{+50}_{-60}$  \\
\quad relative$^{b}$
 & $1.16^{+0.19}_{-0.21}\,\%$ & $25^{+8}_{-8}\,\%$ & $40^{+13}_{-12}\,\%$ & $2.5^{+0.7}_{-0.7}\,\%$  \\
\quad residual$^{c}$
 & $87.7^{+1.9}_{-1.8}\,\%$ & $37^{+18}_{-20}\,\%$ & $38^{+17}_{-19}\,\%$ & $62^{+10}_{-9}\,\%$  \\


==> paramtable.tex <==
$N_\mathrm{H}$
& $10^{22}$\,atoms\,cm$^{-2}$
& $1.648_{-0.027}^{+0.027}$
& $1.720_{-0.026}^{+0.024}$
& $1.642_{-0.027}^{+0.027}$
& $1.732_{-0.023}^{+0.025}$
\\
$F_\mathrm{PL}$\,$^{a}$
& $10^{-9}$\,erg\,s$^{-1}$\,cm$^{-2}$
& $4.54_{-0.18}^{+0.19}$
& $2.45_{-0.05}^{+0.05}$
& $4.65_{-0.15}^{+0.18}$
& $2.41_{-0.05}^{+0.05}$
\\
$\Gamma$
& 
& $0.47_{-0.04}^{+0.04}$
& $0.58_{-0.04}^{+0.04}$
& $0.45_{-0.04}^{+0.04}$
& $0.59_{-0.04}^{+0.04}$
\\
$E_\mathrm{fold}$
& keV
& $10.0_{-0.4}^{+0.5}$
& $9.3_{-0.4}^{+0.4}$
& $10.0_{-0.4}^{+0.5}$
& $9.17_{-0.28}^{+0.39}$
\\
$F_\mathrm{10\,keV}$\,$^{b}$
& $10^{-9}$\,erg\,s$^{-1}$\,cm$^{-2}$
& $1.83_{-0.13}^{+0.12}$
& $1.28_{-0.04}^{+0.04}$
& $1.88_{-0.13}^{+0.13}$
& $1.31_{-0.04}^{+0.04}$
\\
$E_\mathrm{10\,keV}$
& keV
& $8.70_{-0.15}^{+0.16}$
& $8.05_{-0.09}^{+0.08}$
& $8.87_{-0.15}^{+0.16}$
& $8.10_{-0.10}^{+0.09}$
\\
$\sigma_\mathrm{10\,keV}$
& keV
& $3.22_{-0.14}^{+0.14}$
& $3.12_{-0.07}^{+0.07}$
& $3.15_{-0.14}^{+0.14}$
& $3.05_{-0.09}^{+0.09}$
\\
$\mathrm{EW}_\mathrm{Fe\,K\alpha}$
& eV
& $10.5_{-2.7}^{+2.7}$
& $10.1_{-2.8}^{+2.8}$
& $10.1_{-2.7}^{+2.7}$
& $8.5_{-2.6}^{+2.6}$
\\
$E_\mathrm{Fe\,K\alpha}$
& keV
& $6.343_{-0.029}^{+0.035}$
& $6.44_{-0.04}^{+0.06}$
& $6.343_{-0.029}^{+0.035}$
& $6.45_{-0.07}^{+0.04}$
\\
$\mathrm{EW}_\mathrm{Fe\,XXV\,K\alpha}$
& eV
& $13.5_{-3.1}^{+2.9}$
& $8.2_{-3.0}^{+2.6}$
& $13.3_{-3.1}^{+2.9}$
& $6.4_{-2.7}^{+2.7}$
\\
$E_\mathrm{Fe\,XXV\,K\alpha}$
& keV
& $6.641_{-0.030}^{+0.033}$
& $6.73_{-0.09}^{+0.05}$
& $6.642_{-0.030}^{+0.030}$
& $6.73_{-0.10}^{+0.05}$
\\
$\mathrm{EW}_\mathrm{Fe\,XXVI\,K\alpha}$
& eV
& $5.3_{-3.0}^{+3.0}$
& --
& $5.1_{-3.0}^{+3.0}$
& --
\\
$E_\mathrm{Fe\,XXVI\,K\alpha}$
& keV
& $6.91_{-0.08}^{+0.25}$
& --
& $6.91_{-0.08}^{+0.25}$
& --
\\[10pt]
$E_\mathrm{CRSF,0}$
& keV
& 10.19$^{\dag\,c}$
& $10.19_{-0.15}^{+0.15}$
& 10.61$^{\dag\,c}$
& $10.61_{-0.21}^{+0.23}$
\\
$W_\mathrm{CRSF,0}$, $\sigma_\mathrm{CRSF,0}$
& keV, keV
& 2$^{\dag}$
& 2$^{\dag}$
& 2$^{\dag}$
& 2$^{\dag}$
\\
$\tau_\mathrm{CRSF,0}$, $D_\mathrm{CRSF,0}$
& --, keV
& 0.096$^{\dag\,c}$
& $0.096_{-0.012}^{+0.012}$
& 0.56$^{\dag\,c}$
& $0.56_{-0.09}^{+0.09}$
\\
$E_\mathrm{CRSF,1}$
& keV
& $21.0_{-0.8}^{+0.7}$
& $21.4_{-0.5}^{+0.6}$
& $21.5_{-0.8}^{+0.7}$
& $21.7_{-0.6}^{+0.6}$
\\
$W_\mathrm{CRSF,1}$, $\sigma_\mathrm{CRSF,1}$
& keV, keV
& 2$^{\dag}$
& 2$^{\dag}$
& 2$^{\dag}$
& 2$^{\dag}$
\\
$\tau_\mathrm{CRSF,1}$, $D_\mathrm{CRSF,1}$
& --, keV
& $0.10_{-0.05}^{+0.06}$
& $0.115_{-0.029}^{+0.030}$
& $0.41_{-0.22}^{+0.23}$
& $0.45_{-0.14}^{+0.14}$
\\
$E_\mathrm{CRSF,2}$
& keV
& $34.2_{-1.4}^{+1.4}$
& $32.2_{-2.2}^{+4.6}$
& $35.3_{-1.5}^{+1.5}$
& $32.6_{-2.7}^{+5.4}$
\\
$W_\mathrm{CRSF,2}$, $\sigma_\mathrm{CRSF,2}$
& keV, keV
& 4$^{\dag}$
& 4$^{\dag}$
& 4$^{\dag}$
& 4$^{\dag}$
\\
$\tau_\mathrm{CRSF,2}$, $D_\mathrm{CRSF,2}$
& --, keV
& $0.17_{-0.06}^{+0.06}$
& $0.05_{-0.04}^{+0.07}$
& $1.5_{-0.6}^{+0.6}$
& $\le 0.70$
\\
$c_\mathrm{XIS0}$
& 
& $1.023_{-0.004}^{+0.004}$
& $1.007_{-0.004}^{+0.004}$
& $1.023_{-0.004}^{+0.004}$
& $1.007_{-0.004}^{+0.004}$
\\
$c_\mathrm{XIS1}$
& 
& $1.084_{-0.004}^{+0.004}$
& $1.117_{-0.005}^{+0.005}$
& $1.084_{-0.004}^{+0.004}$
& $1.117_{-0.005}^{+0.005}$
\\
$c_\mathrm{PIN}$
& 
& $1.18_{-0.08}^{+0.08}$
& $1.616_{-0.016}^{+0.016}$
& $1.12_{-0.08}^{+0.08}$
& $1.616_{-0.015}^{+0.016}$
\\
$c_\mathrm{PCA}$
& 
& --
& $1.268_{-0.006}^{+0.006}$
& --
& $1.269_{-0.005}^{+0.005}$
\\[10pt]
\multicolumn{2}{l|}{$\chi^2_\mathrm{red}$ / dof}

& 1.29 / 516
& 1.44 / 574
& 1.29 / 516
& 1.51 / 574
\\

